Personalized Generative Models for Contextual Debiasing

Different visual patterns appear with different frequencies in the world: e.g., beach balls appear on sand more often than they do on a road. These statistics are reflected in vision datasets, and as a result trained models more easily recognize objects in common scenarios. However, recognizing a beach ball on a road may arguably be even more important than recognizing it on sand. We study how to mitigate this discrepancy. Since collecting uncommon images in the real world may be difficult, we explore whether generating images with less frequent contexts can serve as effective training augmentation. A key challenge is guiding generations to remain close to the original dataset distribution while creating diverse images with uncommon contexts. We introduce Decoupling Contextual Patterns with Generations (DecoupleGen), a method that personalizes text-to-image diffusion models to facilitate coherent synthesis of images with rare contexts while preserving original visual details. The generated images contain semantically meaningful content and remain visually aligned with the original datasets. We further apply verification constraints to ensure relevance of the augmented data. We evaluate our approach on object classification and recognition tasks on complex scene datasets. Our experiments demonstrate consistent improvements over previous approaches, and our analyses identify factors underlying these improvements.

==> 4page_sections/discussion.tex <==
\vspace{-3mm}
\section{Conclusion}
\vspace{-1mm}
In this work, we introduce \textbf{\proj}, a contextual debiasing pipeline that generate images with out-of-context patterns by adapting personalized Txt2Img models, improving classification and recognition performance while producing visually consistent and semantically aligned samples.

==> 4page_sections/experiments.tex <==
\vspace{-1mm}
\section{Experiments} \label{sec:baseline_coco}

% We set out to generate synthetic images to increase sampling of the underrepresented regions of the dataset, while keeping generations as close to the original training data distribution as possible. Our goal is to increase the accuracy of the models trained with this data augmentation on underrepresented groups while preserving the accuracy on the well represented groups. In this section, we first demonstrate that our method achieves better performance compared to existing work that modifies training objectives on original datasets as well as approaches that leverage generative models to synthesize additional training samples (Section \ref{sec:baseline}). We then provide analysis of potential factors contributing to advantages of our method with respect to alternative generation-based approaches (Section \ref{sec:reason_why}). 

In this section, we evaluate our framework on object recognition task. We include complete experimental setups, results, and analysis in Appendix~\ref{app:exp_extend}.

\begin{table*}[!ht]
    \centering
    % \small
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
        Method & Num Generations & Exclusive mAP & Cooccur mAP & Unbiased mAP & All mAP \\
        \midrule
        Standard & 0 & 24.10 $\pm$ 0.13 & \textbf{64.80} $\pm$ 0.08 & \textbf{72.54} $\pm$ 0.04 & \textbf{55.97} $\pm$ 0.02 \\
        Real Cooccur & 0 & 22.69 $\pm$ 0.53 & 64.00 $\pm$ 0.57 & 71.28 $\pm$ 0.24 & 54.82 $\pm$ 0.31 \\
        Class balancing loss \citep{cui2019class} & 0 & 25.03 $\pm$ 0.06 & 64.67 $\pm$ 0.05 & 72.35 $\pm$ 0.04 & 55.79 $\pm$ 0.02 \\
        Negative penalty \citep{singh2020don} & 0 & 23.71 $\pm$ 0.03 & 64.61 $\pm$ 0.07 & 72.19 $\pm$ 0.05 & 55.68 $\pm$ 0.02 \\
        % Split biased class & 20.60 & 62.39 & 72.46 & 52.15 \\
        Weighted loss \citep{singh2020don} & 0 & \textbf{28.21} $\pm$ 0.15 & 59.89 $\pm$ 0.16 & 72.13 $\pm$ 0.01 & 55.44 $\pm$ 0.00 \\
        Remove cooccur labels \citep{singh2020don} & 0 & 24.17 $\pm$ 0.06 & 64.59 $\pm$ 0.06 & 71.59 $\pm$ 0.04 & 55.30 $\pm$ 0.01 \\
        Remove cooccur images \citep{singh2020don} & 0 & 28.09 $\pm$ 0.34 & 60.09 $\pm$ 0.08 & 72.25 $\pm$ 0.04 & 55.50 $\pm$ 0.04 \\
        CAM \citep{singh2020don} & 0 & 25.09 $\pm$ 0.23 & 64.45 $\pm$ 0.04 & 72.45 $\pm$ 0.04 & 55.87 $\pm$ 0.01 \\ 
        Feature split \citep{singh2020don} & 0 & 26.76 $\pm$ 0.52 & 64.10 $\pm$ 0.01 & 72.39 $\pm$ 0.07 & 55.74 $\pm$ 0.02 \\
        \midrule
        Txt2Img Cooccur \citep{rombach2022high} & $18k$ & 24.66 $\pm$ 0.36 & 64.41 $\pm$ 0.08 & 72.87 $\pm$ 0.14 & 56.11 $\pm$ 0.20 \\
        Txt2Img Exclusive \citep{rombach2022high} & $18k$ & 25.01 $\pm$ 1.04 & 65.26 $\pm$ 0.09 & 72.66 $\pm$ 0.02 & 55.96 $\pm$ 0.04 \\
        Txt2Img Target Class \citep{rombach2022high} & $18k$ & 23.90 $\pm$ 0.40 & 64.87 $\pm$ 0.15 & 72.44 $\pm$ 0.02 & 55.92 $\pm$ 0.02 \\
        SD Inpainting \citep{rombach2022high} & $18k$ & 25.34 $\pm$ 1.13 & 64.77 $\pm$ 0.09 & 72.61 $\pm$ 0.01 & 55.85 $\pm$ 0.05 \\
        Blended LD \citep{avrahami2022blended} & $18k$ & 24.87 $\pm$ 0.57 & 64.77 $\pm$ 0.05 & 72.71 $\pm$ 0.01 & 55.94 $\pm$ 0.01 \\
        Feedback Guidance \citep{hemmat2023feedback} & $18k$ & 25.55 $\pm$ 0.01 & 65.01 $\pm$ 0.06 & 72.68 $\pm$ 0.01 & 56.11 $\pm$ 0.01 \\
        DecoupleGen (ours) & $18k$ & \textbf{27.20} $\pm$ 0.32 & \textbf{65.56} $\pm$ 0.04 & \textbf{73.09} $\pm$ 0.03 & \textbf{56.37} $\pm$ 0.04 \\
        \midrule
        DecoupleGen (ours) & $96k$ & \textbf{29.52} $\pm$ 0.21 & \textbf{66.43} $\pm$ 0.04 & \textbf{73.52} $\pm$ 0.05 & \textbf{57.00} $\pm$ 0.06 \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Quantitative comparisons on COCO dataset.}
    We compare \proj{} performance to methods that modify training objectives on original dataset, where we include all successful generations from our method, totaling 96k in classifier training (top). We also compare \proj{} performance to different generation-based approaches, where we keep the number of additional samples for each target biased class consistent, totaling 18k generations (bottom). \proj{} achieves better performance in all evaluations compared to existing work in both scenarios. The best performance within each block is bolded.}
\label{tab:baseline_coco}
\vspace{-5mm}
\end{table*}

\vspace{-5mm}
\paragraph{Experimental setup.} 
We use COCO-Stuff \citep{caesar2018coco} dataset, which contains complex real-world scene images, for recognition of multiple objects. 
%
\citet{singh2020don} defined a bias score measure to identify biased categories and their co-occurring context; we use the same set of biased classes for evaluations. Our goal is to improve model performance on images where biased classes do not exist together with their common context labels. 

To generate samples that manipulate contextual patterns, we follow the semantic label hierarchy of the original dataset to identify sets of similar categories within the same super class for replacement. We generate 1 output from each replacement or removal prompt to avoid duplicates and encourage diversity in generated semantic contents. We then decide a generation as successful if its annotation label only contains \texttt{b} (target class) without  \texttt{c} (common context label) and only keep the successful generations. This results in 96k generations in total.

We evaluate classifier performance, using average precision (AP) as the metric for each class. We consider several evaluation metrics following previous work \citep{singh2020don}: (1) \textbf{Exclusive mAP} is computed over 20 biased classes on images where  \texttt{b} \textit{never} exists with  \texttt{c}; (2) \textbf{Cooccur mAP} is computed over 20 biased classes on images where  \texttt{b} \textit{always} exists with  \texttt{c}; (3) \textbf{Unbiased mAP} is computed over remaining 60 object classes in COCO; and (4) \textbf{All mAP} is computed over all 171 object and context classes.

\vspace{-5.8mm}
\paragraph{Comparison with loss-function based approaches.}
In addition to the baseline of \textbf{Standard} classifier that is trained on the original dataset with supervised loss, we compare the performance of our method to two sets of previous work. The first set includes approaches that modify training objectives on original datasets in order to improve performance on underrepresented groups. As proposed in \citet{singh2020don}, we consider \textbf{Class balancing loss}, \textbf{Negative penalty}, \textbf{Weighted loss}, \textbf{Remove cooccur labels}, \textbf{Remove coocccur images}, \textbf{CAM}, which uses class activation map \citep{zhou2016cam} as weak location annotation in classifier training, and \textbf{Feature split}, which enforces classifier to learn separate feature space for objects and their context. 

When comparing to these approaches utilizing alternative loss functions, we use all successful generations with uncommon contextual patterns (96k) to augment the original training set in classifier training and report performances in Table~\ref{tab:baseline_coco}~(top half). 
Our method achieves better performance on all evaluation metrics compared to these loss-function based approaches.
We observe $1.3\%$ improvements in exclusive mAP from $28.21\%$ in re-weighting objective to $29.52\%$ in our method, and  $1.6\%$ improvements in cooccur mAP from $64.80\%$ in standard classifier to $66.43\%$ in our method.
While previous approaches reduce performance on cooccur, unbiased, and all mAP metrics to improve performance on exclusive images, our method shows consistent improvements on all evaluation metrics.

\vspace{-5.2mm}
\paragraph{Comparison with other generation-based approaches.} Since our method generates additional training samples for downstream tasks, we compare to several alternative generative approaches. 
\textbf{Txt2Img} with three variants, where captions describing target biased classes we aim to improve (\textbf{Txt2Img Target Class}), co-occurring image (\textbf{Txt2Img Cooccur}), or exclusive images (\textbf{Txt2Img Exclusive}) are used to generate synthetic images \citep{li2023blip, rombach2022high}; \textbf{Feedback Guidance} \citep{hemmat2023feedback} where we use the same captions as Txt2Img Target Class approach, and include guidance from standard classifier since classifier entropy reduces to classification loss in this multi-label classification problem setting; \textbf{Stable Diffusion Inpainting}, which is an inpainting model for local image editing trained to reconstruct masked region from remaining unmasked area \citep{rombach2022high}; and \textbf{Blended Latent Diffusion}, where the editing mask is applied in the down-sampled latent space and masked and unmasked areas are blended together throughout the diffusion process \citep{avrahami2023blended}. 

To compare effectiveness of different generation-based methods, we fix the number of samples added to each target biased class consistent across different baselines, matching those in cooccur images from original dataset (18k in total). This is due to challenges in successfully manipulating contextual labels using local image editing models (we discuss more details in Section \ref{sec:reason_why}). We also perform the same filtering process to only include successful generations on methods that manipulate contextual patterns.

Table \ref{tab:baseline_coco} shows that \proj{} improves on the standard method with 18k images as well, and outperforms other generative data augmentation approaches in all evaluation metrics. The largest improvement is in exclusive mAP; DecoupleGen improves on Feedback Guidance by $1.6\%$ achieving an mAP of $27.2\%$ from $25.6\%$. The improvement on exclusive mAP is especially noteworthy, indicating that our generations provide useful information for underrepresented groups in the dataset. 


==> 4page_sections/introduction.tex <==

\section{Introduction}
\label{sec:intro}

Improvements in computer vision models is fueled, in part, through improvements in data collection methods, resulting in ever-larger datasets. However, despite diverse curation strategies, these datasets still contain biases of multiple forms~\cite{buolamwini2018gender, shankar2017no, birhane2021large, van2016stereotyping, zhao2021understanding}. One way these biases can manifest is through the common co-occurring patterns; for example, skis frequently appear with people, while images of skis alone are rare. 
These \emph{contextual biases} often result in the model failing to generalize to uncommon scenarios; going back to our example, these models often have low accuracy for images of skis without people~\cite{singh2020don}. 
While recent general-purpose vision-language models may exhibit greater robustness to such biases due to large-scale pretraining~\citep{bai2025qwen3,singh2025openai}, our goal is not to replace small classifiers with multimodal foundation models. Many real-world and industrial applications still utilize smaller specialized models given compute and memory constraint~\citep{liao2022kitti,caesar2020nuscenes}, motivating the need to improve generalization of compact classifiers.

\begin{figure}[!t]
    \centering
        \begin{subfigure}[b]{0.24\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/result_hard/20635_orig.pdf}
             \caption{Original}
             \label{fig:pipe_hard_orig}
         \end{subfigure}
        \hspace{-0.02\linewidth}
        \begin{subfigure}[b]{0.24\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/pipe_hard/txt2img.png}
             \caption{Txt2Img~\citep{rombach2022high}}
             \label{fig:pipe_hard_txt2img}
         \end{subfigure}
         \hspace{-0.02\linewidth}
        \begin{subfigure}[b]{0.24\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/result_hard/20635_pretrain.pdf}
             \caption{Inpaint~\citep{rombach2022high}}
             \label{fig:pipe_hard_inpaint}
         \end{subfigure}
        \hspace{-0.02\linewidth}
        \begin{subfigure}[b]{0.24\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/result_hard/20635_finetune_2.pdf}
             \caption{DecoupleGen}
             \label{fig:pipe_hard_ours}
         \end{subfigure}
        \hspace{-0.02\linewidth}
    \caption{\textbf{An example of challenges in contextual debiasing.}
    Our goal is to generate an image of skis without person. Utilizing common Txt2Img models usually generate very different visual appearance from original datasets. Applying existing local image editing models, e.g. inpainting, usually generates images that are less reasonable. Modifying other elements related to person is necessary to ensure visual coherence of the entire image.}
    \label{fig:pipe_hard}
    \vspace{-6mm}
\end{figure}

One way to address these biases is through constructing training objectives, such as reweighting, that penalize models for over-relying on contextual cues~\citep{singh2020don, cui2019class,bickel2009discriminative, fernandez2018cost}. However, these methods are limited to only utilizing original datasets and can often result in poorer performance on in-context samples. 
An alternative way to tackle these biases is through leveraging recent advances in generative models~\cite{rombach2022high, ho2020denoising, nichol2021glide, ramesh2021zero, hertz2022prompt} to synthesize images with diverse contents. These models can be used to edit images to remove the common context, or generate images with difficult contexts. Recent works explore the potential to incorporate these generations as data augmentation to improve recognition performance. However, they usually focus on classification of single object in an image~\citep{azizi2023synthetic, he2022synthetic, dunlap2024diversify, hemmat2023feedback}, thus are not well equipped to handle interactions between multiple objects in real world scenarios, limiting their potential scope and applicability.

Constructing images that contain objects in uncommon contexts through generative models can be challenging. Since objects and scenes usually interact with each other in real images, manipulating contextual patterns requires handling their complex relationships in order to generate natural looking images.
Furthermore, in order for these samples to improve model performance, we would like the resulting generations ideally to be close to the distribution of the original dataset. Consider the COCO~\cite{caesar2018coco} dataset and in particular images containing skis, the person within the image usually interacts with the skis in some way (Figure~\ref{fig:pipe_hard_orig}). When generating images with rare contexts such as skis without people, large-scale pre-trained text-to-image (Txt2Img) models often create images with drastically different viewpoints and backgrounds to that of the original dataset (Figure~\ref{fig:pipe_hard_txt2img}), which may not be relevant to downstream tasks. On the other hand, local editing methods, e.g. inpainting~\citep{rombach2022high, birhane2021large} or blended diffusion~\citep{avrahami2022blended, avrahami2023blended}, which takes mask as input to explicitly remove (or replace) the context, are unable to deal with interactions among objects. Removing the person in this way results in the skis floating (Figure~\ref{fig:pipe_hard_inpaint}).
Instead, generating a version of this image without the person requires that the skis also be repositioned to generate a plausible image, as shown in Figure~\ref{fig:pipe_hard_ours}. 

To address this issue, we introduce our approach for \textbf{Decoupl}ing Cont\textbf{e}xtual Patterns with \textbf{Gen}erations (\textbf{DeoupleGen}) (Figure \ref{fig:pipe_main}). We adapt pre-trained diffusion models to downstream datasets by fine-tuning on every co-occurring image and generate samples containing uncommon contextual partners in training datasets. Specifically, inspired by personalization methods of diffusion models for subject-driven generations \citep{ruiz2023dreambooth, gal2022image}, we learn new word tokens to describe visual details from original images. We then prompt fine-tuned diffusion models with learned text embeddings to manipulate contextual patterns. The resulting generations are natural looking and similar to the images from the original dataset. To utilize meaningful generations more relevant to downstream recognition tasks, we select synthesized images that do not contain common contextual patterns to ensure additional samples used for classifier training capture underrepresented groups in original datasets, thereby supplementing out-of-context samples.

We evaluate \proj{} on real-world object and scene datasets \citep{caesar2018coco, he2021towards}. Our experiments show that \proj{} outperforms existing approaches that modify loss functions or leverage generative models for data augmentation by 1.5\%, and improves from standard classifier trained on original dataset by 5.4\%. Our analyses show two distinctive features of \proj{}: first, synthesized images from \proj{} stay closer to the downstream dataset, indicating better alignment; and second, \proj{} is better capable of accounting for complex relationships between objects and scenes depicted in natural images.
\footnote{In this work, “personalization” refers to subject-driven visual generation techniques that extract and reproduce specific visual concepts from one or a few reference samples.} % ; this is distinct from “personalized agents”~\citep{zhao2025do,pan2025secom} that tailors lanaguage model responses towards user preferences and behaviors
% including additional samples from our method for classifier training


==> 4page_sections/pipeline.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/metadata/pipeline.pdf}
    \caption{\textbf{Overview of DecoupleGen.}
    We first fine-tune text-to-image diffusion models on each co-occurring image by learning new word tokens to describe visual details. We then synthesize images by combining these learned text embeddings to manipulate contextual patterns. Our generations are visually coherent and maintain visual information similar to original image. Finally, we select relevant and meaningful generations via a verification process and incorporate them in classifier training.}
    \label{fig:pipe_main}
    \vspace{-5mm}
\end{figure*}

\vspace{-1mm}
\section{Contextual Debiasing via Generative Model}
We aim to augment the original dataset with generations not containing common contextual patterns, while encouraging these generations to be visually reasonable and close to the original dataset distribution. To achieve this goal, we perform text-to-image generations while maintaining visual information by adapting personalization methods of diffusion models on individual samples.

We propose our method for \textbf{Decoupl}ing Cont\textbf{e}xtual Patterns with \textbf{Gen}erations (\textbf{DecoupleGen}) and provide an overview of the approach in 
Figure \ref{fig:pipe_main}.
Our method consists of three steps: Starting with real images with common contextual patterns, we first fine-tune text-to-image diffusion models to learn new word tokens that describe visual details of different components (biased object, contextual object, background) of these images. We then guide generations to create images without common contextual patterns by composing these learned word tokens. Finally, we filter the synthetic images to remove any images that may still contain common contextual patterns using a pretrained object detector.  
We augment the real dataset with generated images for classifier training.

\vspace{-1mm}
\subsection{Problem Formulation: Image Generation}
We aim to disentangle biased object classes \texttt{b} (e.g., skateboard) from their contextual categories \texttt{c} (e.g., person) by generating images that remove common co-occurrence patterns. Specifically, we formulate contextual debiasing as editing images containing \texttt{(b, c)} by either removing \texttt{c} or replacing it with alternative semantic categories, while preserving the remaining visual content.

\noindent \textbf{What is hard in this problem? }
Images encode complex object–scene relationships, making direct edits prone to producing implausible results (e.g., a floating skateboard). Meanwhile, off-the-shelf text-to-image models often fail to preserve viewpoint and other image-specific details. Our goal is therefore to generate images that reposition objects while maintaining the original visual characteristics.

\vspace{-1mm}
\subsection{Adapting Personalized Diffusion Models} \label{pipe:gen}

We take inspiration from recent personalization methods \citep{ruiz2023dreambooth, gal2022image, kumari2023multi} that fine-tune a special token to reconstruct a subject. Specifically, we train the text encoder to learn a new ``background'' token that captures visual details of the remaining pixels.

\textit{At training time}, given an image with masks of \texttt{b} and \texttt{c}, we associate a new \texttt{[Vbackground]} token to reconstruct visual details specified by remaining pixels not included in either \texttt{b} or \texttt{c}. We provide masks of \texttt{b} and \texttt{c} as input, and background mask is defined to be all remaining pixels not in either class. The word tokens and the diffusion model are optimized to reconstruct the image from the text input ``a photo of \texttt{[Vhandbag]} and \texttt{[Vperson]} and \texttt{[Vbackground]}". Following \citet{avrahami2023break}, we use training objective $\mathcal{L} = \mathcal{L}_{\text{maskrec}} + \lambda \mathcal{L}_{\text{crossattn}}$, where 
\begin{align*}
    \mathcal{L}_{\text{maskrec}} = \mathbf{E}_{z, m, \epsilon, t} 
    \left[ \Vert \epsilon \odot M_m - \epsilon_{\theta} (z, t, \texttt{V}_m ) \odot M_m \Vert ^2 \right]
\end{align*}

is the variational lower bound loss between predicted noise $\epsilon_\theta$, with $z$ being the noisy latent at diffusion timestep $t$, and added noise $\epsilon \sim \mathcal{N}(0, 1)$ that ensures faithful reconstruction of each masked region $M_m$ from text $\texttt{V}_m$ on the $m$-th token and 
\begin{align*}
    \mathcal{L}_{\text{crossattn}} = \mathbf{E}_{z, m, t}
    \left[ \Vert \text{CrossAttn}_\theta (z, t, \texttt{V}_m) - M_m \Vert ^2 \right]
\end{align*}
is cross attention loss that ensures each word token $\texttt{V}_m$ attends only to the corresponding masked region $M_m$ and no other region.

\textit{At inference time}, we generate from finetuned diffusion models by prompting with learned word tokens. Specifically for example, ``a photo of handbag at \texttt{[Vbackground]}" for removing person, and ``a photo of handbag and dog at \texttt{[Vbackground]}" for replacing person with dog, or other alternatives. 

\textit{A verification step} on synthesized samples is helpful, since our approach to manipulate contextual patterns does not guarantee that generations are always successful. After generation, we annotate each image using an off-the-shelf pre-trained semantic segmentation model \citep{jain2023oneformer} and predict class labels. We discard images that do not have the expected labels in the sample selection step. 
For example, given an image with both skateboard and person, successful generations containing skateboard but not person will be included. 
This verification process ensures that generated samples contain information helpful to downstream tasks. 
